Measuring Fluxes of Meteor Showers with the NASA All-Sky Fireball Network

We present an algorithm developed to measure the fluxes of major meteor showers as observed in NASA's All-Sky Fireball Network cameras. Measurements of fluxes from the All-Sky cameras not only improve the Meteoroid Environment Office's (MEO's) ability to provide accurate risk assessments from major showers, but also allows the mass distribution of meteoroids within the shower to be constrained. This algorithm accounts for the shower-specific and event-specific exposure time and collecting area of the sky for nights where sufficiently large samples of shower meteors ($\sim 30$ or more from the shower) are observed. The fluxes derived from the All-Sky Fireball Network for the 2015 Geminid, 2016 Perseid and Quadrantid, 2017 Orionid, and 2018 Leonid shower peaks are calculated. All five of these shower fluxes show excellent agreement with expectations from independent measurements at different mass and luminosity limits. For four of these five showers, the measured mass indices are significantly shallower than what is currently assumed by the NASA Meteoroid Environment Office's (MEO's) annual meteor shower forecast. A direct comparison between forecasted and measured fluxes at limiting masses of $\sim 1 \thinspace \mathrm{g}$ shows good agreement for the three showers for which the observations took place near their peak activity.

==> All Sky Fluxes Arxiv/reference_defs.tex <==
\def \aap {A\&A} % alternative A&A code
\def \statisci {Statis. Sci.}
\def \physrep {Phys. Rep.}
\def \pre {Phys.\ Rev.\ E}
\def \sjos {Scand. J. Statis.} % Scandinavian Journal of Statistics
\def \jrssb {J. Roy. Statist. Soc. B} % Journal of the Royal Statistical Society. Series B (Statistical Methodology)

% note: one of the macros below causes the dvips output to go crazy on the references page
% uncomment as necessary, at your own risk



% This is ASTROMNEMONIC.BIB, a bibliography database file that provides 
% mnmonics for journal names, which can be used in the `journal' field of 
% bibliography entries in databases for BibTeX.
% The abbreviations of the most popular Astronomical journal names in 
% this file are set out in 1993 MNRAS 160, 1. For the other journals,
% the abbreviations of the journal names in this file follow the rules of
% the International List of Periodical Title Word Abbreviations.
% From: Astronomy and Astrophysics Abstracts, 1990, Vol. 49A
% As coded in mnemonic.bib, by Sake J. Hogeveen.
%
% H. Ferguson 19 May 1993

\def \araa {ARA\&A}
% \def \afz {Afz}
\def \aj {AJ}
% \def \azh {AZh}
% \def \aa {A\&A}
 \def \aas {A\&AS}
% \def \aar {A\&AR}
\def \apj {ApJ}
\def \apjl {ApJL}
\def \apjs {ApJS}
 \def \aaps {Ap\&SS}
% \def \baas {BAAS}
% \def \jaa {JA\&A}
\def \mnras {MNRAS}
\def \nat {Nat}
\def \pasj {PASJ}
 \def \pasp {PASP}
% \def \qjras {QJRAS}
% \def \science {Sci}
% \def \sva {SvA}
\def \sovast{Soviet~Ast.}
% \def \aao {AAO Newsl.}
% \def \aavso {AAVSO Newsl.}
% \def \acta {Acta Astron.}
% \def \aaguv {Acta Astron.\ Geophys.\ Univ.\ Comenianae}
% \def \actastsin {Acta Astron.\ Sin.}
% \def \actapsin {Acta Astrophys.\ Sin.}
% \def \agg {Acta Geod.\ Geophys.}
% \def \ags {Acta Geophys.\ Sin.}
% \def \appsb {Acta Phys.\ Pol., Ser.\ B}
% \def \atash {Acta Tech.\ Acad.\ Sci.\ Hung.}
% \def \advp {Adv.\ Phys.}
% \def \advsr {Adv.\ Space Res.}
% \def \aip {AIP Conf.\ Proc.}
% \def \aavsob {Am.\ Assoc.\ Variable Star Obs.\ Bull.}
% \def \aavsoc {Am.\ Assoc.\ Variable Star Obs.\ Circ.}
% \def \amjp {Am.\ J.\ Phys.}
% \def \aatar {Anglo--Aust.\ Telesc., Annu.\ Rep.}
% \def \ag {Ann.\ Geophys.}
% \def \apl {Ann.\ Phys.\ (Leipzig)}
% \def \apny {Ann.\ Phys.\ (N.Y.)}
% \def \app {Ann.\ Phys.\ (Paris)}
% \def \ao {Appl.\ Opt.}
% \def \appl {Appl.\ Phys.\ Lett.}
% \def \apb {Appl.\ Phys., B}
% \def \as {Appl.\ Spectrosc.}
% \def \ahes {Arch.\ Hist.\ Exact Sci.}
% \def \archuk {Archeoastronomy (U.K.)}
% \def \asbts {Archenhold--Sternw.\ Berlin--Treptow, Sonderdr.}
% \def \asbtvs {Archenhold--Sternw.\ Berlin--Treptow, Vortr.\ Schr.}
% \def \aonaicnl {Arecibo Obs./NAIC, Newsl.}
% \def \artsat {Artif.\ Satell.}
% \def \aiisao {Astrofiz.\ Issled.\ Izv.\ Spets.\ Astrofiz.\ Obs.}
% \def \abco {Astron.\ Bull.\ (Carter Obs.)}
% \def \agas {Astron.\ Ges., Abstr.\ Ser.}
% \def \asther {Astron.\ Her.}
% \def \aiubc {Astron.\ Inst.\ Univ.\ Brno, Contrib.}
% \def \an {Astron.\ Nachr.}
% \def \astnow {Astron.\ Now}
% \def \astraum {Astron.\ Raumfahrt}
% \def \astriha {Astron.\ Rechen-Inst.Heidelb., Mitt., Ser.\ A}
% \def \astrihb {Astron.\ Rechen-Inst.Heidelb., Mitt., Ser.\ B}
% \def \astschu {Astron.\ Sch.}
% \def \asttid {Astron.\ Tidsskr.}
% \def \asttsir {Astron.\ Tsirk.}
% \def \astvest {Astron.\ Vestn.}
% \def \astuai {Astronomia UAI}
% \def \astie {Astronomie}
% \def \asty {Astronomy}
% \def \aplc {Astrophys.\ Lett.\ Commun.}
% \def \ap {Astrophysics}
% \def \aanlsor {Atti Accad.\ Naz.\ Lincei, Ser.\ Ottava, Rend.}
% \def \ajast {Aust.\ J.\ Astron.}
% \def \ajp {Aust.\ J.\ Phys.}
% \def \bavm {BAV Mitt.}
% \def \bavr {BAV Rundbrief}
% \def \bbsag {BBSAG Bull.}
% \def \bestarnl {Be Star Newsl.}
% \def \bildw {Bild Wiss.}
% \def \bipm {BIPM Circ.\ T}
% \def \boaumkt {Biul.\ Obs.\ Astron.\ Uniw.\ M.\ Kopernika Toruniu}
% \def \boe {Bol.\ Obs.\ Ebro}
% \def \broa {Bol.\ ROA}
% \def \blm {Boundary-Layer Meteorol.}
% \def \boop {Boyden Obs., Occas.\ Publ.}
% \def \bastac {Br.\ Astron.\ Assoc.\ Circ.}
% \def \bjp {Bulg.\ J.\ Phys.}
% \def \baps {Bull.\ Am.\ Phys.\ Soc.}
% \def \bafoev {Bull.\ Assoc.\ Fr.\ Obs.\ Etoiles Variables}
% \def \bastic {Bull.\ Astron.\ Inst.\ Czech.}
% \def \basi {Bull.\ Astron.\ Soc.\ India}
% \def \bcao {Bull.\ Crimean Astrophys.\ Obs.}
% \def \bgsi {Bull.\ Geogr.\ Surv.\ Inst.}
% \def \bicds {Bull.\ Inf.\ Cent.\ Donn\'ees Stellaires}
% \def \boab {Bull.\ Obs.\ Astron.\ Belgr.}
% \def \crassgvs {C.\ R.\ Acad.\ Sci., S\'er.\ G\'en., Vie Sci.}
% \def \crassii {C.\ R.\ Acad.\ Sci., II}
% \def \cjp {Can.\ J.\ Phys.}
% \def \cm {Celest.\ Mech.}
% \def \cassos {Cent.\ Astron.\ Sci.\ Spat., Obs.\ Sol.}
% \def \cent {Centaurus}
% \def \cpl {Chem.\ Phys.\ Lett.}
% \def \chinaa {Chin.\ Astron.\ Astrophys.}
% \def \chinp {Chin.\ Phys.}
% \def \chinpl {Chin.\ Phys.\ Lett.}
% \def \ciel {Ciel}
% \def \cielt {Ciel Terre}
% \def \ccotl {Circ.\ Czech.\ Obs.\ Time Lattiude}
% \def \cinf {Circ.\ Inf.}
% \def \ctls {Circ.\ Time Latitude Serv.}
% \def \cqg {Classical Quantum Gravity}
% \def \cast {Comments Astrophys.}
% \def \cnpp {Comments Nucl.\ Part.\ Phys.}
% \def \cppcf {Comments Plasma Phys.\ Controlled Fusion}
% \def \cfsua {Commun.\ Fac.\ Sci.\ Univ.\ Ankara, Ser.\ A2, A3}
% \def \cko {Commun.\ Konkoly Obs.}
% \def \cmp {Commun.\ Math.\ Phys.}
% \def \culo {Commun.\ Univ.\ Lond.\ Obs.}
% \def \comp {Comput.\ Phys.}
% \def \compcom {Comput.\ Phys.\ Commun.}
% \def \cp {Contemp.\ Phys.}
% \def \caosp {Contrib.\ Astron.\ Obs.\ Skalnat\'e Pleso}
% \def \cap {Contrib.\ Atmos.\ Phys.}
% \def \cdaut {Contrib.\ Dep.\ Astron., Univ.\ Tokyo}
% \def \clo {Contrib.\ Lick Obs.}
% \def \cncopb {Contrib.\ Nicholas Copernicus Obs.\ Planetarium Brno}
% \def \cnjro {Contrib.\ Nizamiah Japal-Rangapur Obs.}
% \def \cpp {Contrib.\ Plasma Phys.}
% \def \cvvo {Contrib.\ Van Vleck Obs.}
% \def \cr {Cosmic Res.}
% \def \cryo {Cryogenics}
% \def \czjp {Czech.\ J.\ Phys., Sect.\ B}
% \def \drho {Data Rep.\ Hydrogr.\ Obs., Ser.\ Astron.\ Geod.}
% \def \dgkbawb {Dtsch.\ Geod.\ Komm.\ Bayer.\ Akad.\ Wiss., Reihe B}
% \def \dgkbawc {Dtsch.\ Geod.\ Komm.\ Bayer.\ Akad.\ Wiss., Reihe C}
% \def \dgkbawe {Dtsch.\ Geod.\ Komm.\ Bayer.\ Akad.\ Wiss., Reihe E}
% \def \epsl {Earth Planet.\ Sci.\ Lett.}
% \def \erb {Earth Rotation Bull.}
% \def \emp {Earth, Moon, Planets}
% \def \esrev {Earth--Sci.\ Rev.}
% \def \esab {ESA Bull.}
% \def \esaiuenl {ESA IUE Newsl.}
% \def \esaj {ESA J.}
% \def \esoar {ESO Ann.\ Rep.}
% \def \ejp {Eur.\ J.\ Phys.}
% \def \epl {Europhys.\ Lett.}
% \def \epn {Europhys.\ News}
% \def \expast {Exp.\ Astron.}
% \def \fiz {Fizika}
% \def \fortp {Fortschr.\ Phys.}
% \def \fp {Found.\ Phys.}
% \def \funcp {Fundam.\ Cosmic Phys.}
% \def \gaab {G.~A.A.B.}
% \def \gast {G.\ Astron.}
% \def \gem {Gemini}
% \def \grg {Gen.\ Relativ.\ Gravitation}
\def \gca {Geochim.\ Cosmochim.\ Acta}
% \def \ga {Geomagn.\ Aehron.}
% \def \gafd {Geophys.\ Astrophys.\ Fluid Dyn.}
% \def \gj {Geophys.\ J.}
% \def \grl {Geophys.\ Res.\ Lett.}
% \def \geo {Geophysics}
% \def \geos {GEOS Circ.}
% \def \gbg {Gerlands Beitr.\ Geophys.}
% \def \heav {Heavens}
% \def \hpa {Helv.\ Phys.\ Acta}
% \def \hepnp {High Energ.\ Phys.\ Nucl.\ Phys.}
% \def \hob {Hvar Obs.\ Bull.}
% \def \hi {Hyperfine Interact.}
% \def \iappp {I.A.P.P.P.\ Commun.}
% \def \iauc {IAU Circ.}
% \def \iauib {IAU Inf.\ Bull.}
 \def \icarus {Icarus}
% \def \i3etm {IEEE Trans.\ Magn.}
% \def \i3etns {IEEE Trans.\ Nucl.\ Sci.}
% \def \i3etps {IEEE Trans.\ Plasma Sci.}
% \def \iersbb {IERS Bull.\ B}
% \def \iersba {IERS Bull.--A}
% \def \ijpap {Indian J.\ Pure Appl.\ Phys.}
% \def \ijrsp {Indian J.\ Radio Space Phys.}
% \def \ibvs {Inf.\ Bull.\ Variable Stars}
% \def \iaatub {Inst.\ Astron.\ Astrophys.\ Tech.\ Univ.\ Berlin, Mitt.}
% \def \iag {Inst.\ Astron.\ Geod., Univ.\ Madr., Publ.}
% \def \ia {Inst.\ Astron., Univ.\ Camb., Annu.\ Rep.}
% \def \icq {Int.\ Comet Q.}
% \def \ijimw {Int.\ J.\ Infrared Millimeter Waves}
% \def \ijmp {Int.\ J.\ Mod.\ Phys.\ A}
% \def \ijtp {Int.\ J.\ Theor.\ Phys.}
% \def \ip {Inverse Probl.}
% \def \iastj {Ir.\ Astron.\ J.}
% \def \iris {IRIS Bull.\ A}
% \def \iskz {Issled.\ Solntsa Krasnykh Zvezd}
% \def \intsa {Itogi Nauki Tekh., Ser.\ Astron.}
% \def \intsppk {Itogi NAuki Tekh., Ser.\ Plazmennye Protsessy Kosmose}
% \def \iaoe {Izv.\ Astron.\ Obs.\ Ehngel'gardt.}
% \def \ikao {Izv.\ Krym.\ Astrofiz.\ Obs.}
% \def \ivuzr {Izv.\ Vyssch.\ Uchebn.\ Zaved., Radiofiz.}
% \def \jasa {J.\ Acoust.\ Soc.\ Am.}
% \def \jaavso {J.\ Am.\ Assoc.\ Variable Star Obs.}
% \def \jam {J.\ Appl.\ Meteorol.}
% \def \jap {J.\ Appl.\ Phys.}
% \def \jastf {J.\ Astron.\ Fr.}
% \def \japast {J.\ Astrophys.\ Astron.}
% \def \jas {J.\ Atmos.\ Sci.}
% \def \jatp {J.\ Atmos.\ Terr.\ Phys.}
% \def \jbasta {J.\ Br.\ Astron.\ Assoc.}
% \def \jbis {J.\ Br.\ Interplanet.\ Soc.}
% \def \jcp {J.\ Chem.\ Phys.}
% \def \jcomp {J.\ Comp.\ Phys.}
% \def \jel {J.\ Electrostat.}
% \def \jfseu {J.\ Fac Sci., Ege Univ., Ser.\ A}
% \def \jfm {J.\ Fluid Mech.}
% \def \jgr {J.\ Geophys.\ Res.}
% \def \jhast {J.\ Hist.\ Astron.}
% \def \jms {J.\ Mater.\ Sci.}
% \def \jmp {J.\ Math.\ Phys.}
% \def \jmo {J.\ Mod.\ Opt.}
% \def \jop {J.\ Opt.\ (Paris)}
% \def \josaa {J.\ Opt.\ Soc.\ Am.\ A}
% \def \josab {J.\ Opt.\ Soc.\ Am.\ B}
% \def \jp {J.\ Phys.}
% \def \jpa {J.\ Phys.\ A}
% \def \jpb {J.\ Phys.\ B}
% \def \jpd {J.\ Phys.\ D}
% \def \jpe {J.\ Phys.\ E}
% \def \jpg {J.\ Phys.\ G}
% \def \jpsj {J.\ Phys.\ Soc.\ Jpn.}
% \def \jpp {J.\ Plasma Phys.}
% \def \jqsrt {J.\ Quant.\ Spectrosc.\ Radiat.\ Transfer}
% \def \jrasc {J.\ R.\ Astron.\ Soc.\ Can.}
% \def \jsp {J.\ Stat.\ Phys.}
% \def \jvst {J.\ Vac.\ Sci.\ Technol., A}
% \def \jetpl {JETP Lett.}
% \def \jhatd {Johns Hopkins APL Tech.\ Dig.}
% \def \jjap1 {Jpn.\ J.\ Appl.\ Phys., Part 1}
% \def \jjap2 {Jpn.\ J.\ Appl.\ Phys., Part 2}
% \def \kai {Kapteyn Astron.\ Inst., Annu.\ Rep.}
% \def \kexto {Kexue Tongbao}
% \def \kfnt {Kinematika Fiz.\ Nebesn.\ Tel}
% \def \kob {Kodaikanal Obs.\ Bull.}
% \def \kt {Komet.\ Tsirk.}
% \def \ki {Kosm.\ Issled.}
% \def \koz {Kozmos}
% \def \kpm {KPM}
% \def \lo {Laser Optoelektron.}
% \def \latc {Latitude Circ.}
% \def \lest {LEST Found., Annu.\ Rep.}
% \def \lmp {Lett.\ Math.\ Phys.}
% \def \lob {Lick Obs.\ Bull.}
% \def \mg {Manuscr.\ Geod.}
% \def \ml {Mater.\ Lett.}
% \def \mrb {Mater.\ Res.\ Bull.}
% \def \mfs {Mem.\ Fac.\ Sci., Kyoto Univ., Ser.\ Phys., Astrophys., Geophys., Chem.}
% \def \msai {Mem.\ Soc.\ Astron.\ Ital.}
% \def \merc {Mercury}
% \def \mess {Messenger}
% \def \met {Meteoritics}
% \def \metka {Meteoritika}
% \def \metro {Metrologica}
% \def \mpb {Minor Planet Bull.}
% \def \mpc {Minor Planet Circ.}
% \def \masbt {Mitt.\ Archenold--Sternw.\ Berlin Treptow}
% \def \mag {Mitt.\ Astron.\ Ges.}
% \def \mlotud {Mitt.\ Lohrmann--Obs., Tech.\ Univ.\ Dresden}
% \def \mss {Mitt.\ Sternw.\ Sonneberg}
% \def \mvs {Mitt.\ Ver{\a}nderliche Sterne"}
% \def \mzpe {Mitt.\ Zentralinst.\ Phys.\ Erde}
% \def \mpla {Mod.\ Phys.\ Lett.\ A}
% \def \mnassa {Mon.\ Notes Astron.\ Soc.\ S.\ Afr.}
% \def \nint {Nablyud.\ Iskusstv.\ Nebesn.\ Tel.}
% \def \nogb {Nachr.\ Olbers--Ges.\ Bremen}
% \def \naoj {Natl.\ Astron.\ Obs.\ (Jpn.), Repr.}
% \def \ng {Natl.\ Geogr.}
% \def \nraoa {Natl.\ Radio Astron.\ Obs., Repr., Ser.\ A}
% \def \nraob {Natl.\ Radio Astron.\ Obs., Repr., Ser.\ B}
% \def \natwis {Naturwissenschaften}
% \def \ni {Nauchn.\ Inf.}
% \def \nlasny {News Lett.\ Astron.\ Soc.\ N.Y.}
% \def \nrodaour {Nizamiah Rangapur Obs.\ Dep.\ Astron., Osmania Univ., Repr.}
% \def \nraow {NRAO Workshop}
% \def \nimpra {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ A}
% \def \nimprb {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ B}
% \def \npa {Nucl.\ Phys.\ A}
% \def \npb {Nucl.\ Phys.\ B, Part.\ Phys.}
% \def \nca {Nuovo Cimento A}
% \def \ncb {Nuovo Cimento B}
% \def \ncc {Nuovo Cimento C}
% \def \ot {Obs.\ Trav.}
% \def \obs {Observatory}
% \def \onl {Occultation Newsl.}
% \def \ozvp {{\O}sterr.\ Z.\ Vermessungswes.\ Photogramm."}
% \def \oc {Opt.\ Commun.}
% \def \oe {Opt.\ Eng.}
% \def \olt {Opt.\ Laser Technol.}
% \def \ol {Opt.\ Lett.}
% \def \on {Opt.\ News}
% \def \os {Opt.\ Spectrosc.}
% \def \optik {Optik}
% \def \ofeb {Origins Life Evol.\ Biosphere}
% \def \orion {Orion}
% \def \orione {Orione}
% \def \oac {Oss.\ Astrofis.\ Catania, Pubbl.}
% \def \pz {Perem.\ Zvezdy}
% \def \pb {Phys.\ Bl.}
% \def \pcm {Phys.\ Chem.\ Miner.}
% \def \pfa {Phys.\ Fluids, A}
% \def \pfb {Phys.\ Fluids, B}
% \def \pla {Phys.\ Lett.\ A}
% \def \plb {Phys.\ Lett.\ B}
% \def \pr {Phys.\ Rep.}
% \def \pra {Phys.\ Rev.\ A}
% \def \prb {Phys.\ Rev.\ B}
% \def \prc {Phys.\ Rev.\ C}
\def \prd {Phys.\ Rev.\ D}
\def \prl {Phys.\ Rev.\ Lett.}
% \def \ps {Phys.\ Scr.}
% \def \ptch {Phys.\ Teach.}
% \def \ptod {Phys.\ Today}
% \def \pha {Physica A}
% \def \phb {Physica B}
% \def \phd {Physica D}
% \def \paz {Pis'ma Astron.\ Zh.}
\def \pss {Planetary \& Space Science }
\def \planss {Planetary \& Space Science}
% \def \ppcf {Plasma Phys.\ Controlled Fusion}
% \def \pa {Postepy Astron.}
% \def \pram {Pram\~{a}na}
% \def \pri {Priroda}
% \def \pasa {Proc.\ Astron.\ Soc.\ Aust.}
% \def \pi3e {Proc.\ IEEE}
% \def \prsl {Proc.\ R.\ Soc.\ London, Ser.\ A}
% \def \posp {Proceedings of SPIE}
% \def \past {Prog.\ Astron.}
% \def \ptp {Prog.\ Theor.\ Phys.}
% \def \paicas {Publ.\ Astron.\ Inst.\ Czech.\ Acad.\ Sci.}
% \def \pbao {Publ.\ Beijing Astron.\ Obs.}
% \def \pdaub {Publ.\ Dep.\ Astron., Univ.\ Beogr.}
% \def \pdao {Publ.\ Dom.\ Astrophys.\ Obs.}
% \def \pnlaoj {Publ.\ Natl.\ Astron.\ Obs.\ Jpn.}
% \def \ppmo {Publ.\ Purple Mt.\ Obs.}
% \def \psao {Publ.\ Shaanxi Astron.\ Obs.}
% \def \pscds {Publ.\ Sp\'ec.\ Cent.\ Donn\'ees Stellaires}
% \def \pyo {Publ.\ Yunnan Obs.}
% \def \pag {Pure Appl.\ Geophys.}
% \def \qbsa {Q.\ Bull.\ Sol.\ Act.}
% \def \rad {Radiant}
% \def \rsci {Radio Sci.}
% \def \reche {Recherche}
% \def \rpp {Rep.\ Prog.\ Phys.}
% \def \ra {Rev.\ Astron.}
% \def \rg {Rev.\ Geophys.}
% \def \rmf {Rev.\ Mex.\ Fis.}
% \def \rmp {Rev.\ Mod.\ Phys.}
% \def \rrp {Rev.\ Roum.\ Phys.}
% \def \rsi {Rev.\ Sci.\ Instrum.}
% \def \rnc {Riv.\ Nuovo Cimento}
% \def \rh {\v{R}\'{\i}\v{s}e hv\v{e}zd}
% \def \saaoar {S.\ Afr.\ Astron.\ Obs., Annu.\ Rep.}
% \def \saaoc {S.\ Afr.\ Astron.\ Obs., Circ.}
% \def \saaon {SAAO Newsl.}
% \def \sciam {Sci.\ Am.}
% \def \scch {Sci.\ China, Ser.\ A}
% \def \srtu {Sci.\ Rep.\ T\^{o}hoku Univ., Eighth Ser.}
% \def \sc {Science}
% \def \sar {Sendai Astron.\ Rap.}
% \def \st {Sidereal Times}
% \def \sky {Sky Telesc.}
% \def \sbaavso {Sol.\ Bull.\ (AAVSO)}
% \def \se {Sol.\ Energy}
% \def \sp {Sol.\ Phys.}
% \def \srd {Sol.\ Radio Data}
% \def \ssres {Sol.\ Syst.\ Res.}
% \def \sdb {Soln.\ Dannye, Byull.}
% \def \sonne {Sonne}
% \def \sbo {Soobshch.\ Byurak.\ Obs.}
% \def \ssao {Soobshch.\ Spets.\ Astrofiz.\ Obs.}
% \def \sost {South.\ Stars}
% \def \sal {Sov.\ Astron.\ Lett.}
% \def \sjot {Sov.\ J.\ Opt.\ Technol.}
% \def \spd {Sov.\ Phys.\ -- Dokl.}
% \def \spj {Sov.\ Phys.\ -- JETP}
% \def \spu {Sov.\ Phys.\ -- Usp.}
% \def \space {Space}
% \def \ssr {Space Sci.\ Rev.}
% \def \stsi {Space Telesc.\ Sci.\ Inst., Newsl.}
% \def \sf {Spaceflight}
% \def \sterne {Sterne}
% \def \sw {Sterne Weltraum}
% \def \sb {Sternenbote}
% \def \strlast {Strolling Astron.}
% \def \sgg {Stud.\ Geophys.\ Geod.}
% \def \taot {Tartu Astrof{\u}{\"u}s.\ Obs.\ Teated"}
% \def \tect {Tectonophysics}
% \def \tellus {Tellus, Ser.\ A}
% \def \tmf {Teor.\ Mat.\ Fiz.}
% \def \tp {Theor.\ Pap.}
% \def \tsb {Time Serv.\ Bull.}
% \def \tmnr {Tokyo Meteor Network Rep.}
% \def \tai {Tsirk.\ Astron.\ Inst.\ (Tashkent)}
% \def \ufz {Ukr.\ Fiz.\ Zh.}
% \def \ucla {Universe Classroom}
% \def \uao {Upps.\ Astron.\ Obs., Rep.}
% \def \urania {Urania}
% \def \usnoc {U.S.\ Nav.\ Obs., Circ.}
% \def \usnos4 {U.S.\ Nav.\ Obs., Ser.\ 4}
% \def \ufn {Usp.\ Fiz.\ Nauk}
% \def \vsb {Variable Star Bull.}
% \def \vasiona {Vasiona}
% \def \varih {Ver{\o}ff.\ Astron.\ Rechen--Inst.\ Heidelb."}
% \def \vzpe {Ver{\o}ff.\ Zentralinst.\ Phys.\ Erde"}
% \def \vesmir {Vesm\'{\i}r}
% \def \vansssr {Vestn.\ Akad.\ Nauk SSSR}
% \def \vku {Vestn.\ Kiev.\ Univ., Astron.}
% \def \va {Vistas Astron.}
% \def \wgn {WGN}
% \def \wztud {Wiss.\ Z.\ Tech.\ Univ.\ Dresden}
% \def \yama {Yamamoto Circ.}
% \def \zamp {Z.\ Angew.\ Math.\ Phys.}
% \def \zna {Z.\ Naturforsch., A}
% \def \zpa {Z.\ Phys., A}
% \def \zpc {Z.\ Phys., C}
% \def \zv {Zemlya Vselennaya}
% \def \zenit {Zenit}
% \def \zetf {Zh.\ Ehksp.\ Teor.\ Fiz.}


==> All Sky Fluxes Arxiv/units.tex <==
% 	Simple u\mathrmnits
\def\arcsec{{\mathrm{\thinspace arcsec}}}
\def\cm{{\mathrm{\thinspace cm}}}
\def\erg{{\mathrm{\thinspace erg}}}
\def\eV{{\mathrm{\thinspace eV}}}
\def\g{{\mathrm{\thinspace g}}}
\def\mg{{\mathrm{\thinspace mg}}}
\def\kg{{\mathrm{\thinspace kg}}}
\def\G{{\mathrm{\thinspace G}}}
\def\J{{\mathrm{\thinspace J}}}
\def\ga{{\mathrm{\thinspace gauss}}}
\def\Jy{{\mathrm{\thinspace Jy}}}
\def\K{{\mathrm{\thinspace K}}}
\def\keV{{\mathrm{\thinspace keV}}}
\def\MeV{{\mathrm{\thinspace MeV}}}
\def\km{{\mathrm{\thinspace km}}}
\def\kpc{{\mathrm{\thinspace kpc}}}
\def\Lsun{\hbox{$\mathrm{\thinspace L_{\odot}$}}}
\def\m{{\mathrm{\thinspace m}}}
\def\mm{{\mathrm{\thinspace mm}}}
\def\mJy{{\mathrm{\thinspace mJy}}}
\def\Mpc{{\mathrm{\thinspace Mpc}}}
\def\Msun{\hbox{$\mathrm{\thinspace M_{\odot}$}}}
\def\Rsun{\hbox{$\mathrm{\thinspace R_{\odot}$}}}
\def\pc{{\mathrm{\thinspace pc}}}
\def\ph{{\mathrm{\thinspace ph}}}
\def\s{{\mathrm{\thinspace s}}}
\def\hr{{\mathrm{\thinspace hr}}}
\def\yr{{\mathrm{\thinspace yr}}}
\def\Zsun{\hbox{$\mathrm{\thinspace Z_{\odot}$}}}
\def\Lstar{\hbox{$\mathrm{\thinspace L^{\star}$}}}
\def\sr{{\mathrm{\thinspace sr}}}
\def\Hz{{\mathrm{\thinspace Hz}}}
\def\MHz{{\mathrm{\thinspace MHz}}}
%	Compound units
\def\cmps{\hbox{$\cm\s^{-1}\,$}}
\def\cmsq{\hbox{$\cm^2\,$}}
\def\flux{\hbox{$\keV\cm^{-2}\s^{-1}\sr^{-1}\keV^{-1}\,$}}
\def\col{\hbox{$\cm^{-2}\,$}}
\def\ergcmcups{\hbox{$\erg\cm^3\ps\,$}}
\def\ergpcmps{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\def\ergpcmsqps{\hbox{$\erg\cm^{-2}\s^{-1}\,$}}
\def\ergpcmsqpspAparcsecsq{\hbox{$\erg\cm^{-2}\s^{-1}\AA^{-1}\arcsec^{-2}\,$}}
\def\ergpcmpspsr{\hbox{$\erg\cm^{-2}\s^{-1}\sr^{-1}\,$}}
\def\ergpcmpspsrpHz{\hbox{$\erg\cm^{-2}\s^{-1}\sr^{-1}\Hz^{-1}\,$}}
\def\ergps{\hbox{$\erg\s^{-1}\,$}}
\def\gpcm{\hbox{$\g\cm^{-3}\,$}}
\def\gpcmps{\hbox{$\g\cm^{-3}\s^{-1}\,$}}
\def\gps{\hbox{$\g\s^{-1}\,$}}
\def\kmps{\hbox{$\km\s^{-1}\,$}}
\def\kmps{\hbox{$\km\s^{-1}\,$}}
\def\kmphr{\hbox{$\km\hr^{-1}\,$}}
\def\kmkmphr{\hbox{$\km^{-2}\hr^{-1}\,$}}
\def\Lsunppc{\hbox{$\Lsun\pc^{-3}\,$}}
\def\Msunpc{\hbox{$\Msun\pc^{-3}\,$}}
\def\Msunpkpc{\hbox{$\Msun\kpc^{-1}\,$}}
\def\Msunppc{\hbox{$\Msun\pc^{-3}\,$}}
\def\Msunppcpyr{\hbox{$\Msun\pc^{-3}\yr^{-1}\,$}}
\def\Msunpyr{\hbox{$\Msun\yr^{-1}\,$}}
\def\pcm{\hbox{$\cm^{-3}\,$}}
\def\pcmK{\hbox{$\cm^{-3}\K$}}
\def\phpcmsqps{\hbox{$\ph\cm^{-2}\s^{-1}\,$}}
\def\pHz{\hbox{$\Hz^{-1}\,$}}
\def\ps{\hbox{$\s^{-1}\,$}}
\def\psqcm{\hbox{$\cm^{-2}\,$}}
\def\psr{\hbox{$\sr^{-1}\,$}}
\def\pyr{\hbox{$\yr^{-1}\,$}}
\def\kmpspMpc{\hbox{$\kmps\Mpc^{-1}$}}
\def\Msunpyrpkpc{\hbox{$\Msunpyr\kpc^{-1}$}}

